A phase-field approach for modeling equilibrium solute segregation at the interphase boundary in binary alloys

A number of experimental and theoretical findings in age hardening alloys suggest that specific solute elements preferentially segregate to and reduce the energy of the interphase boundary (IB). This segregation mechanism can stabilize the precipitation microstructure against coarsening, allowing higher operating temperatures in structural applications. Herein, we present a phase field model of solute segregation to IBs that separate matrix and precipitate phases in binary alloys. The proposed modeling framework is capable of capturing bulk thermodynamics and interfacial free energies, while also accounting for various mass transport mechanisms. Analytical equilibrium solutions of one-dimensional systems are presented, and excess IB quantities are evaluated independent of the Gibbs dividing surface convention. With the aid of the parallel tangent construction, IB segregation isotherms are established in terms of the alloy composition and the model parameters describing the free energy functions. Under the regular solution approximation, computational studies elucidating the dependence of the IB energy and segregation levels on temperature and free energy model parameters are presented. We show that the model is consistent with the Gibbs adsorption equation; therefore, it is possible to compare the adsorption behavior predicted by the model parameters with experiments and atomistic simulations. Future work on extending the model to ternary alloys, and incorporating the effect of elastic interactions on IB segregation is expected.

==> Figures/wbm_model/equilibrium_properties.tex <==
\section{Equilibrium Properties}

\subsection{Phase-Field Profile}

\begin{align} \label{eq:steady-state_c}
    \frac{\delta F}{\delta c} = \left. \frac{\partial f_{mix}}{\partial c} \right|_{c_e} + g(\phi_e)\frac{d W}{dc_e} = \mu_c^e \textrm{ (const.)}
\end{align}

\begin{align} \label{eq:steady-state_phi}
    \frac{\delta F}{\delta \phi} = \left. \frac{\partial f_{mix}}{\partial \phi} \right|_{\phi_e} - \epsilon^2  \frac{d^2 \phi_e}{d x^2}  = 0
\end{align}

Integrating the second equality in Eq. \ref{eq:steady-state_c} from $c_e^\alpha$ to $c_e^\beta$ results in,
% Common tangent construction:
\begin{align} \label{eq:common_tgt}
    \mu_c^e = \frac{f_\beta(c_e^\beta)-f_\alpha(c_e^\alpha)}{c_e^\beta-c_e^\alpha} =  \left.\frac{\partial f_{\alpha}}{\partial c} \right|_{c_e^\alpha}
\end{align}

i.e. the compositions of bulk phases $c_e^\alpha$ and $c_e^\beta$ satisfy the common tangent construction.

\begin{align} \label{eq:ce_phie_double_derv}
    \frac{\partial^2 f}{\partial c_e^2} dc_e + \frac{\partial^2 f}{\partial c_e \partial \phi_e} d\phi_e = 0
\end{align}

% \begin{equation} \label{eq:ce_phie_fn_reln}
% \resizebox{0.5\linewidth}{!}{$
% \frac{dc_e}{d\phi_e} = \frac{h^{\prime}(\phi_e)\left(\frac{\partial f^\alpha}{\partial c_e} - \frac{\partial f^\beta}{\partial c_e}\right) - g^{\prime}(\phi_e)\frac{\partial W}{\partial c_e}}{[1-h(\phi_e)]\frac{\partial^2 f^\alpha}{\partial c_e^2} + h(\phi_e) \frac{\partial^2 f^\beta}{\partial c_e^2} + g(\phi_e)\frac{\partial^2 W}{\partial c_e^2}}
% $}\end{equation}

\begin{equation} \label{eq:ce_phie_RS_reln}
\resizebox{0.9\linewidth}{!}{$
\frac{dc_e}{d\phi_e} = \frac{\left[G_\beta^B - G_\beta^A - G_\alpha^B + G_\alpha^A + (\Omega_\beta - \Omega_\alpha)(1-2c_e) \right]h^\prime(\phi_e) + \left[W_B-W_A+W_{AB}(1-2c_e)\right]g^{\prime}(\phi_e)}
    {2\Omega_\alpha + 2(\Omega_\beta-\Omega_\alpha) h(\phi_e) + 2W_{AB}g(\phi_e) - RT/[V_m(1-c_e)c_e]}
$}\end{equation}

\begin{align} \label{eq:phie_profile}
    \frac{\epsilon^2}{2} \left(\frac{d\phi_e}{dx}\right)^2 =& f(c_e,\phi_e) - f_\alpha(c_e^\alpha) - \left.\frac{\partial f_\alpha}{\partial c}\right|_{c_e^\alpha}(c_e - c_e^\alpha)
\end{align}

\begin{align} \label{eq:ce_profile}
    \frac{dc_e}{dx} = \frac{dc_e}{d\phi_e}\frac{d\phi_e}{dx}
\end{align}

Eqs. \ref{eq:phie_profile} and \ref{eq:ce_profile} are solved simultaneously to obtain $\phi_e(x)$ and $c_e(x)$.

% \begin{align}
%     \frac{\delta F}{\delta \phi} = \left[f_{\beta}(c_e)-f_{\alpha}(c_e)\right] \left.\frac{\partial h}{\partial \phi_e}\right|_{\phi_e} + W(c_e)\frac{dg}{d\phi_e} - \epsilon^2 \frac{d^2 \phi_e}{d x^2} = 0
% \end{align}

% \begin{align}
%     \frac{\delta F}{\delta c} = [1-h(\phi_e)]\left.\frac{\partial f_{\alpha}}{\partial c}\right|_{c_e} + h(\phi_e)\left.\frac{\partial f_{\beta}}{\partial c}\right|_{c_e} + g(\phi_e)\left.\frac{\partial W}{\partial c} \right|_{c_e} = \mu_c^e \textrm{ (const.)}
% \end{align}



% \begin{align*}
%     \frac{\delta F}{\delta \phi} = \left[f_{\beta}(c_e)-f_{\alpha}(c_e)\right] \left.\frac{\partial h}{\partial \phi_e}\right|_{\phi_e} + W(c_e)\frac{dg}{d\phi_e} - \epsilon^2 \frac{d^2 \phi_e}{d x^2} = 0
% \end{align*}

% \begin{align*}
%     \epsilon \frac{d^2\phi_e}{dx^2} = \left[f_{\beta}(c_e)-f_{\alpha}(c_e)\right]\frac{dh}{d\phi_e} + W(c_e)\frac{dg}{d\phi_e}
% \end{align*}

\subsection{Interface Segregation}

% For $\phi \rightarrow 0$,

\begin{align} \label{eq:steady-state_c_seg}
    \left. \frac{\partial f(c_e,\phi_e)}{\partial c_e} \right. = \left.\frac{\partial f_\alpha}{\partial c}\right|_{c_e^\alpha}
\end{align}

where, $f(c_e,\phi_e)$ is obtained from Eq. \ref{eq:f_local_form2}

The condition for equilibrium is a constant diffusion potential $\mu_c^e$ throughout the system. Graphically, this condition can be represented by the parallel tangent construction as shown in Fig. \ref{fig:RS_param,free_energy}b. The equilibrium phase compositions $c_e^\alpha$ and $c_e^\beta$ are obtained by imposing the condition for equal chemical potentials $\mu_A^e$ and $\mu_B^e$ in the phases; graphically, the compositions satisfy the common tangent condition. The slope of the tangent lines in Fig. \ref{fig:RS_param,free_energy}b is the diffusion potential $\mu_c^e$ and the contact points of tangent lines with the free energy curves are the equilibrium concentrations. The equilibrium concentration at the interface center was obtained from the segregation isotherm (Eq. \ref{eq:seg_isotherm}) for $\phi_e=0.5$.

\begin{align} \label{eq:seg_isotherm}
     \frac{c_e(x)}{1-c_e(x)} = \frac{c_e^\alpha}{1-c_e^\alpha} \exp\left(\frac{\Delta H^{\alpha}_{seg}}{RT/V_{m}}\right)
\end{align}

where,
\begin{align} \label{eq:deltaHseg}
    \Delta H^{\alpha}_{seg} &= G_\alpha^B - G^B(\phi_e) - G_\alpha^A + G^A(\phi_e) + (1-2c_e^\alpha)\Omega_\alpha - (1-2c_e)\Omega(\phi_e) % - 2\Omega_\alpha c_e^\alpha + 2\Omega(\phi_e)c_e  
\end{align}

Interface excess concentration described in terms of Gibbs' diving surface is given by

\begin{align} \label{eq:excess_reln}
    \Gamma_B = C - C_0 = \int_{-L}^{+L} c_e(x) dx - \int_{-L}^{0}c_\alpha^e dx - \int_{0}^{+L}c_\beta^e dx
\end{align}
where, $x = 0$ is chosen as the location of the diving surface. $+L$ and $-L$ are chosen far from the interface. $C_0$ is the total concentration of the reference system with a sharp interface and equilibrium bulk-phase concentrations on either side of the interface (shown in dotted line in Fig. \ref{fig:phase-field_profile}a.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/free_energy_curves.png}
%     \caption{}
%     \label{fig:free_energy}
% \end{figure}

\subsection{Interface Energy and Width}

\begin{align} \label{eq:gamma_int}
    \gamma = \int_{-L}^{L} \epsilon^2 \left(\frac{d\phi_e}{dx}\right)^2 dx
    = \int_{0}^{1} \epsilon^2 \left(\frac{d\phi_e}{dx}\right) d\phi_e
\end{align}

\begin{align} \label{eq:width_int}
    \omega = \int_{0.05}^{0.95} \frac{dx}{d\phi_e} d\phi_e
\end{align}




% \begin{equation*}
%     F = \int \left(f_{ch}(c,\phi) + \frac{\epsilon}{2}\abs{\nabla \phi}^2\right) d\vec{r}
% \end{equation*}

% At steady state,

% \begin{align*}
%     \frac{\delta F}{\delta c} &= \mu_c^e (\textrm{const.}) \\
%     \frac{\delta F}{\delta \phi} &= 0
% \end{align*} \\
    
% where, $\mu_c^e$ is the diffusion potential.

% \subsubsection{Segregation isotherm}

% From the steady-state relation for concentration field,

% \begin{align*}
%     \frac{\delta F}{\delta c} = [1-h(\phi_e)]\left.\frac{\partial f_{\alpha}}{\partial c}\right|_{c_e} + h(\phi_e)\left.\frac{\partial f_{\beta}}{\partial c}\right|_{c_e} - (W_1+2W_2 c_e)g(\phi_e) = \mu_c^e
% \end{align*}

% For $\phi \rightarrow 0$,

% \begin{align*}
%     \left.\frac{\partial f_{\alpha}}{\partial c} \right|_{c^{\alpha}_e} &= \mu_c^e 
%     = G^B_\alpha - G^A_\alpha + \Omega_\alpha (1-2c_e^\alpha) + RT/V_{m} \log \left({\frac{c_e^{\alpha}}{1-c_e^{\alpha}}} \right)
% \end{align*}

% % (NOTE: I'm assuming that the far-field matrix concentration is equal to the equilibrium concentration $c_m^e$ set for the matrix free energy)

% Substituting above, in previous equation,

% \begin{align*}
%     [1-h(\phi_e)]\left.\frac{\partial f_{\alpha}}{\partial c}\right|_{c_e} + h(\phi_e)\left.\frac{\partial f_{\beta}}{\partial c}\right|_{c_e} - (W_1+2W_2 c_e)g(\phi_e) = G^B_\alpha - G^A_\alpha + \Omega_\alpha (1-2c_e^\alpha) + RT/V_{m} \log \left({\frac{c_e^{\alpha}}{1-c_e^{\alpha}}} \right)
% \end{align*}

% Substituting the derivatives of the free energies,

% \begin{align*}
%     & [1-h(\phi_e)]\left[G^B_\alpha - G^A_\alpha + \Omega_{\alpha}(1-2c_e) + RT/V_{m} \log \left(\frac{c_e}{1-c_e}\right)\right] \\
%     & + h(\phi_e)\left[G^B_\beta - G^A_\beta + \Omega_{\beta}(1-2c_e) + RT/V_{m} \log \left(\frac{c_e}{1-c_e}\right)\right] - (W_1+2W_2c_e) g(\phi_e) \\
%     &= G^B_\alpha - G^A_\alpha + \Omega_\alpha (1-2c_e^{\alpha}) + RT/V_m \log \left(\frac{c_e^{\alpha}}{1-c_e^{\alpha}} \right)
% \end{align*}

% This gives,

% \begin{align*}
%      \frac{c_e}{1-c_e} = \frac{c_e^\alpha}{1-c_e^\alpha} \exp\left(\frac{\Delta H_{seg}}{RT/V_{m}}\right)
% \end{align*}

% where,
% \begin{align*}
%     \Delta H_{seg} &= 2\Omega_\alpha(c_e-c_e^\alpha) + (W_1+2W_2c_e)g(\phi_e) \\
%     &- \left[(G^B_\beta-G^B_\alpha)-(G^A_\beta-G^A_\alpha)+(1-2c_e)(\Omega_\beta-\Omega_\alpha)\right] h(\phi_e)   
% \end{align*}

% Taylor expanding the exponential part with respect to $c_e$ about zero, yields a polynomial of $\mathcal{O}(c_e^3)$:

% \begin{align*}
%     \frac{pq^2}{2}c_e^3 + pq\left(1-\frac{q}{2}\right)c_e^2 + (1+p-pq)c_e - p = 0
% \end{align*}

% where,
% \begin{align*}
%     p &= \frac{c_e^\alpha}{1-c_e^\alpha}\exp\left(\frac{-2\Omega_\alpha c_e^\alpha + W_1g(\phi_e) - \left(G^B_\beta - G^A_\beta - G^B_\alpha + G^A_\alpha + \Omega_\beta- \Omega_\alpha \right)h(\phi_e)}{RT/V_m}\right) \\
%     q &= \frac{2\Omega_\alpha+2W_2g(\phi_e)+2(\Omega_\beta-\Omega_\alpha)h(\phi_e)}{RT/V_m}
% \end{align*}

% At the interface centre, i.e. $c_i^e = c_e(\phi_e=0.5)$,

% \begin{align*}
%      \frac{c_e^i}{1-c_e^i} = \frac{c_e^\alpha}{1-c_e^\alpha} \exp\left(\frac{\Delta H^i_{seg}}{RT/V_{m}}\right)
% \end{align*}

% where,

% \begin{align*}
%     \Delta H^i_{seg} &= W_1 + (2W_2+\Omega_\alpha+\Omega_\beta)c_e^i - 2\Omega_\alpha c_e^\alpha \\
%     &\hspace{0.5 cm} -\frac{1}{2}\left[(G^B_\beta-G^B_\alpha)-(G^A_\beta-G^A_\alpha)+(\Omega_\beta-\Omega_\alpha) \right]
% \end{align*}

% % For $W_1 = 0$,

% % \begin{align*}
% %     c_i^e = \frac{1}{2}(c_m^e+c_p^e) + \frac{W_1}{2f_{\alpha}^{''}}
% % \end{align*}

% \subsubsection{Coupling between $c_e$ and $\phi_e$}

% From

% \begin{align*}
%     \frac{\partial f_{ch}(c_e,\phi_e)}{\partial c} = \mu_c^e
% \end{align*}

% we can write the following

% \begin{align*}
%     \frac{\partial^2 f_{ch}}{\partial c_e^2} dc_e + \frac{\partial^2 f_{ch}}{\partial c_e \partial \phi_e} d\phi_e = 0
% \end{align*}

% This relation can be used to derive the coupling between $c_e$ and $\phi_e$ as:

% % \begin{align*}
% %     c_e(\phi_e) = [1-h(\phi_e)]c_e^m + h(\phi_e)c_e^p
% % \end{align*}

% % In the interface segregation model with $W_2 = 0$,

% % \begin{align*}
% %     c_e(\phi_e) = [1-h(\phi_e)]c_e^m + h(\phi_e)c_e^p + \frac{W_1}{2f_{\alpha}^{\prime\prime}} g(\phi_e)
% % \end{align*}

% % For $W_1 \neq 0$ and $W_2 \neq 0$, the following ODE holds:

% \begin{align*}
%     \frac{dc_e}{d\phi_e} = \frac{\left(G^B_\beta-G^B_\alpha - G^A_\beta+G^A_\alpha + (\Omega_\beta-\Omega_\alpha)(1-2c_e) \right)\frac{dh}{d\phi_e} - (W_1+2W_2)\frac{dg}{d\phi_e}}{2\Omega_\alpha - \frac{RT/V_m}{c_e(1-c_e)} - 2(\Omega_\beta-\Omega_\alpha)h(\phi_e) - 2W_2g(\phi_e)}
% \end{align*}

% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{figures/W1_segregation_parametric_plot.png}
% %     \caption{Equilibrium concentration $c_e$ as a function of $\phi_e$ for interface segregation model with $W_2 = 0$. $c_e^m = 0.01$, $c_e^p = 0.33$.}
% %     \label{fig:my_label}
% % \end{figure}

% \subsubsection{Equilibrium phase-field profiles}

% Now consider 

% \begin{align*}
%     \frac{\delta F}{\delta \phi} = \left.\frac{\partial f_{ch}}{\partial \phi} \right|_{\phi_e} - \epsilon \frac{d^2 \phi_e}{d x^2} = 0
% \end{align*}

% \begin{align*}
%     \epsilon \frac{d^2\phi_e}{dx^2} = [f_{\beta}(c_e)-f_{\alpha}(c_e)]\frac{dh}{d\phi_e} + (W_{\phi}^{\prime} - W_1 c_e - W_2 c_e^2)\frac{dg}{d\phi_e}
% \end{align*}

% where, $W_{\phi}^\prime = W_\phi + W_0$. Multiplying both sides with $\frac{d\phi_e}{dx}$ and integrating with respect to $x$ from $-\infty$ to some $x'$, followed by change in variable of integration appropriately,

% \begin{align*}
%     \frac{\epsilon}{2} \left(\frac{d\phi_e}{dx}\right)^2 = \int_0^{\phi_e} W_{\phi}^{\prime}dg(\phi_e) + \int_{c_e^\alpha}^{c_e} [f_{\beta}(c_e)-f_{\alpha}(c_e)]\frac{dh(\phi_e(c_e))}{dc_e}dc_e - \int_{c_e^\alpha}^{c_e} (W_1 c_e + W_2 c_e^2)\frac{dg(\phi_e(c_e))}{dc_e}dc_e
% \end{align*}

% Integrating by-parts the second and third terms on right hand side,

% \begin{align*}
%     \frac{\epsilon}{2} \left(\frac{d\phi_e}{dx}\right)^2 =&  W_{\phi}^{\prime}g(\phi_e) + [f_{\beta}(c_e)-f_{\alpha}(c_e)]h(\phi_e) - (W_1c_e + W_2c_e^2)g(\phi_e) \\ &- \int_{c_e^\alpha}^{c_e} \left(\left(\frac{df_{\beta}}{dc_e}-\frac{df_{\alpha}}{dc_e}\right)h(\phi_e(c_e)) - (W_1 + 2W_2c_e)g(\phi_e(c_e)) \right) dc_e
% \end{align*}

% From the steady-state relation for concentration, the integrand in the above equation can be replaced as:

% \begin{align*}
%     \frac{\epsilon}{2} \left(\frac{d\phi_e}{dx}\right)^2 =& [f_{\beta}(c_e)-f_{\alpha}(c_e)]h(\phi_e) + (W_{\phi}^{\prime}- W_1c_e - W_2c_e^2)g(\phi_e) - \int_{c_e^\alpha}^{c_e} \left(\mu_c^e - \frac{\partial f_{\alpha}}{\partial c_e}  \right) dc_e
% \end{align*}

% This reduces to,

% \begin{align*}
%     \frac{\epsilon}{2} \left(\frac{d\phi_e}{dx}\right)^2 =& f_{ch}(c_e,\phi_e) - f_\alpha(c_e^\alpha) - \left.\frac{\partial f_\alpha}{\partial c}\right|_{c_e^\alpha}(c_e - c_e^\alpha)
% \end{align*}

% The profile for $c_e$ can be described by:

% \begin{align*}
%     \frac{dc_e}{dx} = \frac{dc_e}{d\phi_e}\frac{d\phi_e}{dx}
% \end{align*}

% The steady-state phase-field profiles $\phi_e(x)$ and $c_e(x)$ can be obtained by simultaneously solving $\frac{d\phi_e}{dx}$ and $\frac{dc_e}{dx}$.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/phase_free_energy_material03a_seg01.png}
%     \caption{}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figures/material03a_seg01_phie_validation_new.png}
% %         \caption{Lorem ipsum}
%     \end{subfigure}%
%     ~ ~    
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figures/material03a_seg01_ce_validation_new.png}
% %         \caption{Lorem ipsum}
%     \end{subfigure}%
%     \caption{Parameters: $(G_\alpha^A, G_\alpha^B, \Omega_\alpha)$ = $(0,0,-0.1)$, $(G_\beta^A, G_\beta^B, \Omega_\beta)$ = $(0.2,0.2,-1.5)$, $(W_\phi,\epsilon,RT/V_m)$ = $(0.2,10,0.1)$. Case without segregation: $(W_0,W_1,W_2)$ = $(0,0,0)$; with segregation $(W_0,W_1,W_2)$ = $(0,0.3,0)$. } 
%     % \label{fig:param_T}
% \end{figure} 

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figures/material03a_phie_profiles.png}
% %         \caption{Lorem ipsum}
%     \end{subfigure}%
%     ~ ~    
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figures/material03a_ce_profiles.png}
% %         \caption{Lorem ipsum}
%     \end{subfigure}%
%     \caption{Parameters: $(G_\alpha^A, G_\alpha^B, \Omega_\alpha)$ = $(0,0,-0.1)$, $(G_\beta^A, G_\beta^B, \Omega_\beta)$ = $(0.2,0.2,-1.5)$, $(W_\phi,\epsilon,RT/V_m)$ = $(0.2,10,0.1)$.} 
%     % \label{fig:param_T}
% \end{figure} 

% \subsection{Description}

% In the conventional phase-field approach the energetics of the interface is described by interpolating the free energy functions of the matrix and the precipitate. In this work, we prescribe a distinct free enregy function for the interface center. The term $W_1c + W_2c^2$ describes the devation in the interface free energy function from that given by the two-phase model.

% Describing the composition and interfacial energy of the "planar interphase boundary" is the main objective of this study. For this purpose, we focus on a binary component system as it yields simple analytic relations. Out work will focus on two important properties of the interface: its free energy and composition. These interfacial properties significantly determine precipitation-related aspects like morphology, coarsening kinetics and mechanical properties of the material.

% There have been attempts to describe interphase segregation in the past. Some studies have used "single layer" models to describe the interface, where the interface constitutes a single atomic layer. In these, the interface is treated as a "phase" [my paper?], which is not in agreement with classical thermodynamical definition of an interface. There is diffuse interface model for a ternary system, given by Dregia and Wynblatt: limitations of this?

% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{figures/Numerical_phie.png}
% %     \caption{$\phi_e$ vs. spatial position evaluated numerically for the following parameters: $W_\phi^{'} = 0.2, \epsilon = 5$, $c_e^m = 0.01, c_e^p = 0.33$, $f_{\alpha}^{''} = 1$.}
% %     \label{fig:my_label}
% % \end{figure}

% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.5\textwidth]{figures/Numerical_ce_vs_z.png}
% %     \caption{$c_e$ vs. spatial position evaluated numerically for the following parameters: $W_\phi^{'} = 0.2, \epsilon = 5$, $c_e^m = 0.01, c_e^p = 0.33$, $f_{\alpha}^{''} = 1$.}
% %     \label{fig:my_label}
% % \end{figure}

% \newpage
% \subsubsection{Interfacial energy}

% Interfacial energy is given by (Ref: Lupis, Provatas, WBM),

% \begin{align*}
%     \gamma = \Delta F - (\Gamma_1 \mu_1^e + \Gamma_2 \mu_2^e)
% \end{align*}

% where, $\Delta F$ is the excess free energy per unit area of the interface, $\Gamma_A$ and $\Gamma_B$ are the interface excess concentrations of the components. $\Gamma_B$ is defined by:

% \begin{align*}
%     \Gamma_2 = \int_{-L}^{L} c_e(x) dx - \int_{-L}^{0}c_\alpha^e dx - \int_{0}^{L}c_\beta^e dx
% \end{align*}

% $\Gamma_1 = -\Gamma_2$ for equal molar volumes of $A$ and $B$. Therefore,

% \begin{align*}
%     \gamma = \Delta F - \Gamma_2 \mu_c^e
% \end{align*}

% where,

% \begin{align*}
%     \Delta F =& \int_{-L}^{0} \left(f_{ch}(c_e,\phi_e)+\frac{\epsilon}{2}\left(\frac{d\phi_e}{dx}\right)^2 \right) dx - \int_{-L}^{0} f_{ch}(c_\alpha^e,0) dx \\
%     &+ \int_{0}^{L} \left(f_{ch}(c_e,\phi_e)+\frac{\epsilon}{2}\left(\frac{d\phi_e}{dx}\right)^2 \right) dx - \int_{-L}^{0} f_{ch}(c_\beta^e,1) dx
% \end{align*}

% \begin{align*}
%     \Delta F = \int_{-L}^{0} \left(\epsilon \left(\frac{d\phi_e}{dx}\right)^2 + \mu_c^e(c_e-c_\alpha^e) \right) dx + \int_{0}^{L} \left(\epsilon \left(\frac{d\phi_e}{dx}\right)^2 + \mu_c^e(c_e-c_\beta^e) \right) dx
% \end{align*}

% Therefore,

% \begin{align*}
%     \gamma = \Delta F =& \int_{-L}^{L} \epsilon \left(\frac{d\phi_e}{dx}\right)^2 dx
%     = \int_{0}^{1} \epsilon \left(\frac{d\phi_e}{dx}\right) d\phi_e \\
%     % =& \sqrt{2\epsilon} \int_{0}^{1} \sqrt{f_{ch}(c_e,\phi_e)} d\phi_e
% \end{align*}

% % % \begin{figure}[ht]
% % %     \centering
% % %     \includegraphics[width=0.5\textwidth]{figures/Interfacial_energy_vs_Solute_excess_plot.png}
% % %     \caption{Interfacial energy vs. solute excess evaluated numerically for interface segregation model with $W_2 = 0$, $W_\phi = 1, \epsilon = 1$, $c_e^m = 0.01, c_e^p = 0.33$. $\Gamma_\phi = \int_0^1 c_e(\phi_e)d\phi_e - 0.5(c_m^e+c_p^e) = \frac{4W_1}{15f_{\alpha}^{\prime \prime}}$}
% % %     \label{fig:my_label}
% % % \end{figure}

% % % \newpage


% % % \begin{figure}[ht]
% % %     \centering
% % %     \includegraphics[width=0.5\textwidth]{figures/Simulation_ce_vs_phie.png}
% % %     \caption{}
% % %     \label{fig:my_label}
% % % \end{figure}

% % % \begin{figure}[ht]
% % %     \centering
% % %     \includegraphics[width=0.5\textwidth]{figures/Simulation_ce_vs_distance.png}
% % %     \caption{}
% % %     \label{fig:my_label}
% % % \end{figure}

% \section{KKS model}
% \subsection{Chemical free energy density}

% \begin{align*}
%     f(c,\phi) = f_\alpha(c_\alpha)[1-h(\phi)] + f_\beta (c_\beta) h(\phi) + W(c_\delta)g(\phi)  
% \end{align*}

% where, $c_\alpha = c_\alpha (c,\phi)$, $c_\beta = c_\beta (c,\phi)$, $c_\delta = c_\delta (c, \phi)$ are variables.

% Local concentration is given by

% \begin{align*}
%     c = c_\alpha [1-h(\phi)] + c_\beta h(\phi) + c_\delta g(\phi)
% \end{align*}

% Differentiating with respect to $c$ and $\phi$ yields the following relations:

% \begin{align*}
%     1 &= \frac{\partial{c_\alpha}}{\partial c}[1-h(\phi)] + \frac{\partial{c_\beta}}{\partial c}h(\phi) + \frac{\partial{c_\delta}}{\partial c} g(\phi) \\
%     0 &= \frac{\partial{c_\alpha}}{\partial \phi}[1-h(\phi)] - c_\alpha h^{\prime}(\phi) + \frac{\partial{c_\beta}}{\partial \phi}h(\phi) + c_\beta h^{\prime}(\phi) + \frac{\partial{c_\delta}}{\partial \phi}g(\phi) - c_\delta g^{\prime}(\phi)
% \end{align*}

% Differentiating $f(c,\phi)$ with respect to $c$:

% \begin{align*}
%     f(c,\phi) &= \frac{\partial f_\alpha(c_\alpha)}{\partial c}[1-h(\phi)] + \frac{\partial f_\beta (c_\beta)}{\partial c} h + \frac{\partial W(c_\delta)}{\partial c}g(\phi)   \\
%     &= \frac{\partial f_\alpha(c_\alpha)}{\partial c_\alpha}\frac{\partial c_\alpha}{\partial c}[1-h(\phi)] + \frac{\partial f_\beta (c_\beta)}{\partial c_\beta}\frac{\partial c_\beta}{\partial c} h + \frac{\partial W(c_\delta)}{\partial c_\delta}\frac{\partial c_\alpha}{\partial c} g(\phi)
% \end{align*}

% Imposing the condition:
% \begin{align*}
%     \frac{\partial f_\alpha(c_\alpha)}{\partial c_\alpha} = \frac{\partial f_\beta(c_\beta)}{\partial c_\beta} = \frac{\partial W(c_\delta)}{\partial c_\delta}
% \end{align*}
